Learning to Walk and Fly with Adversarial Motion Priors

Robot multimodal locomotion encompasses the ability to transition between walking and flying, representing a significant challenge in robotics. This work presents an approach that enables automatic smooth transitions between legged and aerial locomotion. Leveraging the concept of Adversarial Motion Priors, our method allows the robot to imitate motion datasets and accomplish the desired task without the need for complex reward functions. The robot learns walking patterns from human-like gaits and aerial locomotion patterns from motions obtained using trajectory optimization. Through this process, the robot adapts the locomotion scheme based on environmental feedback using reinforcement learning, with the spontaneous emergence of mode-switching behavior. The results highlight the potential for achieving multimodal locomotion in aerial humanoid robotics through automatic control of walking and flying modes, paving the way for applications in diverse domains such as search and rescue, surveillance, and exploration missions. This research contributes to advancing the capabilities of aerial humanoid robots in terms of versatile locomotion in various environments.

==> tex/method_old.tex <==
\section{Methodo}
\label{sec:method}


The goal of our work is to train a policy $\pi$ that is capable of walking and flying. This policy should be capable of imitating the locomotion pattern extracted from $k$ locomotion datasets $\mathcal{D}$. Moreover, this policy should choose the best locomotion pattern required to fulfill a task; hence, it should not follow a specific motion.

We model the task as a Markov Decision Process (MDP) defined by a tuple $(\mathcal{S}, \mathcal{A}, \mathcal{P}, r, \rho_0, \gamma)$~\cite{SuttonRichardSBartoReinforcementLearning}. The agent is initialized in a state $s_t \in \mathcal{S}$ from an initial distribution $\rho_0$. An action $a_t \in \mathcal{A}$ is sampled from a stochastic policy $\pi_\theta(a_t|s_t)$ and executed by the agent that hence transitions from the state $s_t$ to the state $s_{t+1}$ with a probability )$\mathcal{P}^{a_t}_{s_t, s_{t+1}} = \text{Pr}(s_{t+1}|s_t, a_t)$, receiving a reward $r(t) \in \mathbb{R}$.

The goal of Deep Reinforcement Learning (DRL) is to find the optimal set of parameters $\theta$ of a neural network policy $\pi_\theta: \mathcal{S} \rightarrow \mathcal{A}$ that maximize the expected discounted return
\begin{equation}
    J(\theta)~=~\mathbb{E}_{\pi_\theta} \left[\sum_{t=0}^{T-1} \gamma^t r(t) \right],
\end{equation}
where $\gamma \in [0, 1)$ is the discount factor that penalizes trading off long-term against short-term rewards.

\subsection{Adversarial Motion Priors}

As in AMP~\cite{peng2021amp}, the reward $r$ is composed of two terms:
\begin{equation}
    r = w_{\text{G}}r_{\text{G}} +w_{\text{S}}r_{\text{S}}.
\end{equation}
The task reward $r_{\text{G}}$ specifies the goal the agent should accomplish, e.g., reach a target or have a desired base velocity. The style reward $r_{\text{S}}$, on the other hand, enforces the policy to produce locomotion patterns resembling the motion of the dataset. The total reward encourages the agent to imitate a desired set of motion patterns, choosing the best to achieve the desired goal.
Given the environment, no high-level planner must select a specific motion, and the switching behavior emerges naturally. \looseness=-1

The style reward $r_G$ is a function of the output of a discriminator $D(s_t,s_{t+1})$. The discriminator $D(s_t,s_{t+1})$ learns to differentiate samples from the motion dataset from samples produced by the RL agent and is trained using the objective proposed in~\cite{peng2021amp, peng2022ase}
\begin{equation}
    \begin{split}
        \operatorname*{arg\,min}_\theta \ & -\mathbb{E}_{(s_t,s_{t+1})\sim\mathcal{D}}[\log(D(s_t,s_{t+1}))] \\
        & - \mathbb{E}_{(s_t,s_{t+1})\sim\mathcal{\pi_\theta}}[\log (1 - D(s,s'))] \\
        & + w_{\text{gp}} \mathbb{E}_{(s_t,s_{t+1})\sim\mathcal{D}} \big [ || \nabla_\Phi D(s_t,s_{t+1})||^2],
    \end{split}
\end{equation}
where the first two terms encourage the discriminator to distinguish if a state transition $(s_t, s_{t+1})$ comes from the motion dataset or the environment. This formulation forces the discriminator to output 1 when the discriminator is fed with dataset transitions and 0 when it is fed with samples produced by the agent. The final term is a gradient penalty that penalizes nonzero gradients on dataset transition. This penalty results in improved stability and quality of the training.

\subsubsection{Style-reward}

The tuple $(s_t, s_{t+1})$ motion produced by the agent is used to compute the syle reward
\begin{equation}
    r_\text{S} = -\log{\Big(1 - \dfrac{1}{1 + e^{D(s_t, s_{t+1})}}\Big)}.
\end{equation}
and rewards the agent when it produces a transition similar to the datasets.

\begin{figure}[t]
    \centering
    \includegraphics[width=1.0\linewidth]{images/ironcubAMP.pdf}
    \caption{AMP scheme: the discriminator outputs a reward with a higher value if the motions of the agent are close to the dataset. The task reward specifies which goal the agent has to aim for.}
    \label{fig:AMP-scheme}
\end{figure}

\subsubsection{Task-reward}

We want the robot to reach a target and follow a route made of checkpoints. Ideally, we could reward the agent when it hits the target. This approach makes associating a reward with an individual action complex since it introduces reward sparsity. A common practice is to use proxy rewards that guide the agent to the true objective and provide continuous feedback to the agent. We use three reward functions to hit the checkpoints and follow the route.

At each time instant, the agent can be associated with a checkpoint. First, we want to minimize the distance of the robot base to the target. This reward is written as:
\begin{equation}
    r_c(t) = a \exp(-b \| x_d - p_t\|^2),
\end{equation}
where $x_d \in \mathbb{R}^3$ represents the target position.

We want the robot to approach the target with a desired velocity $v_d \in \mathbb{R}$. This reward translates in
\begin{equation}
    r_v(t) = a \exp \Big(b\Big\|v_d - \frac{d(p_t) - d(p_{t-1})}{\Delta t}\Big\|^2\Big)
\end{equation}
where $d(p) = \| p - x_d\|$ is a function that computes the scalar distance of the robot base to the target and forces the robot to travel at speed $v_dv_d$ on the base-to-target line.

The last reward demands the agent to face the checkpoint, i.e., to point its $x$-axis to the projection of the target on the horizontal plane:
\begin{equation}
    r_f(t) = \min(0, f(p_t)_{xy} \cdot {}^\asFrame{I}i_{xy})
\end{equation}
where $f(p) = \frac{x_d - p}{\| x_d - p \|}$ computes the unit vector that points from the robot base to the checkpoint, the subscript $xy$ extracts the horizontal components, and the unit vector ${}^\asFrame{I}i{}^\asFrame{I}i$ is the robot $x$-axis in the inertial frame.

Finally, the total task reward is written as
\begin{equation}
    r_{\text{G}} = w_c r_c + w_v r_v + w_f r_f,
\end{equation}
where $w_c, w_v, w_f \in [0,1]$ are weighting each contribution.

%\subsection{Model}
\subsection{Action and Observation Space}


As action space, we choose
\begin{equation}
    a = [s_d, T]
\end{equation}
where $s_d \in \mathbb{R}^n$ are desired joint positions that are fed to a PD control ad $T \in \mathbb{R}^m$ are the desired thrust intensities that act on the mm$m$ specified links and generate a pure force as
\begin{equation}
    f_i = R_i(q) \begin{bmatrix}
        0 \\ 0 \\ -T_i
    \end{bmatrix}, \forall i \in [1, m],
    \label{eq:thrust-force}
\end{equation}
where $R_i(q)$ represents the orientation of the frame on which the force is applied.



Sec~\ref{sec:floating-base} recalls the quantities that describe and act on the system's evolution. We extract some components to build our observation and action space. The observation space consists of two components: one relates to the robot and one distillate information about the task and the environment. We define the robot observation vector as
\begin{equation}
    \mathbf{o}_\text{robot} = [
    \rho, \ {}^\asFrame{B}v_\asFrame{B}, \ {}^\asFrame{B}\omega_\asFrame{B}, \ s, \ \dot{s}, \ ee, \ T
    ]
\end{equation}
where $\rho$ is the quaternion representation of the rotation of the base, ${}^\asFrame{B}v_\asFrame{B}, {}^\asFrame{B}\omega_\asFrame{B}$ is the base velocity in the base frame, $s, \dot{s}$ are the joints position and velocity and $ee$ is the vector containing the position of the end effectors, namely hands and feet, and $T$ is the thrust acting on the system as specified in~\eqref{eq:thrust-force}.

The environment observation vector consists of measurements of the ground height with respect to the base (TODO: rephrase!):
\begin{equation}
    \mathbf{o}_\text{env} = \text{heightmap}
\end{equation}

The task observation specifies where the checkpoint is w.r.t. to the robot:
\begin{equation}
    \mathbf{o}_\text{task} = {}^\asFrame{B}p_\asFrame{T} = {}^\asFrame{I}R_\asFrame{B}^\top (x_d - p)
\end{equation}


\subsubsection{Discriminator Observations}

The discriminator provides feedback about the agent's behavior, telling the policy if it is imitating the motion dataset. Selecting a meaningful set of features to feed into the discriminator is pivotal.
The state transitions $o_t, o_{t+1}$ (\giuseSays{I know, I have to change the notation!}) is passed to an observations map $\Phi(o)$ that extracts:
\begin{equation}
    \Phi(o) = [\rho, \ {}^\asFrame{B}v_\asFrame{B}, \ {}^\asFrame{B}\omega_\asFrame{B}, \ s, \ \dot{s}, \ ee, \ T].
\end{equation}

